End-to-end Mapping in Heterogeneous Systems Using Graph Representation Learning

To enable heterogeneous computing systems with autonomous programming and optimization capabilities, we propose a unified, end-to-end, programmable graph representation learning (PGL) framework that is capable of mining the complexity of high-level programs down to the universal intermediate representation, extracting the specific computational patterns and predicting which code segments would run best on a specific core in heterogeneous hardware platforms. The proposed framework extracts multi-fractal topological features from code graphs, utilizes graph autoencoders to learn how to partition the graph into computational kernels, and exploits graph neural networks (GNN) to predict the correct assignment to a processor type. In the evaluation, we validate the PGL framework and demonstrate a maximum speedup of 6.42x compared to the thread-based execution, and 2.02x compared to the state-of-the-art technique.

==> sec-abstract.tex <==
\begin{abstract}
To enable heterogeneous computing systems with autonomous programming and optimization capabilities, we propose a \emph{unified, end-to-end, programmable graph representation learning} (PGL) framework that is capable of mining the complexity of high-level programs down to the universal intermediate representation, extracting the specific computational patterns and predicting which code segments would run best on a specific core in heterogeneous hardware platforms. %By efficiently representing high-level programs as weighted graphs of universal intermediate representation (IR) instructions working with virtual registers of a universal memory model, the proposed framework can efficiently analyze the structural information flow of software programs and determine their parallelization. Furthermore, 
The proposed framework extracts multi-fractal topological features from code graphs, utilizes graph autoencoders to learn how to partition the graph into computational kernels, and exploits graph neural networks (GNN) to predict the correct assignment to a processor type. In the evaluation, we validate the PGL framework and demonstrate a maximum speedup of 6.42x compared to the thread-based execution, and 2.02x  compared to the state-of-the-art technique.

\end{abstract}
